Accelerated co-design of robots through morphological pretraining

The co-design of robot morphology and neural control typically requires using reinforcement learning to approximate a unique control policy gradient for each body plan, demanding massive amounts of training data to measure the performance of each design. Here we show that a universal, morphology-agnostic controller can be rapidly and directly obtained by gradient-based optimization through differentiable simulation. This process of morphological pretraining allows the designer to explore non-differentiable changes to a robot's physical layout (e.g. adding, removing and recombining discrete body parts) and immediately determine which revisions are beneficial and which are deleterious using the pretrained model. We term this process "zero-shot evolution" and compare it with the simultaneous co-optimization of a universal controller alongside an evolving design population. We find the latter results in diversity collapse, a previously unknown pathology whereby the population -- and thus the controller's training data -- converges to similar designs that are easier to steer with a shared universal controller. We show that zero-shot evolution with a pretrained controller quickly yields a diversity of highly performant designs, and by fine-tuning the pretrained controller on the current population throughout evolution, diversity is not only preserved but significantly increased as superior performance is achieved.

==> 3_results_fig_zero_shot_transfer.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.65\columnwidth]{figs/zero-shot-transfer.pdf}
    \vspace{-8pt}
    \caption{\textbf{fig title}
    fig caption}
    % \vspace{-8pt}
    \label{fig:results-zero-shot-transfer}
\end{figure*}

==> 5_Code.tex <==
\section*{Code}
\label{sec:code}

Code is temporarily withheld to maintain anonymity during review and will be made available upon publication.



==> 6_Impact_Statement.tex <==
\section*{Impact Statement}
\label{sec:impact}

The goal of this paper is to advance the competence and diversity of intelligent robots.
There are numerous potential benefits
and societal consequences of robots,
% \cite{lin2014robot}, 
none which we feel must be specifically highlighted here.

% This work advances automated robot control and design through universal, robot-agnostic control. There are numerous potential benefits such as enabling rapid development of more capable robotic systems for beneficial applications. We acknowledge, however, that robot automation, and automation of robot design, poses risks such as 
% labor displacement and deployment safety concerns.

% Authors are \textbf{required} to include a statement of the potential 
% broader impact of their work, including its ethical aspects and future 
% societal consequences. This statement should be in an unnumbered 
% section at the end of the paper (co-located with Acknowledgements -- 
% the two may appear in either order, but both must be before References), 
% and does not count toward the paper page limit. In many cases, where 
% the ethical impacts and expected societal implications are those that 
% are well established when advancing the field of Machine Learning, 
% substantial discussion is not required, and a simple statement such 
% as the following will suffice:

% ``This paper presents work whose goal is to advance the field of 
% Machine Learning. There are many potential societal consequences 
% of our work, none which we feel must be specifically highlighted here.''

% The above statement can be used verbatim in such cases, but we 
% encourage authors to think about whether there is content which does 
% warrant further discussion, as this statement will be apparent if the 
% paper is later flagged for ethics review.
